Natural Language Interfaces for Spatial and Temporal Databases: A Comprehensive Overview of Methods, Taxonomy, and Future Directions

The task of building a natural language interface to a database, known as NLIDB, has recently gained significant attention from both the database and Natural Language Processing (NLP) communities. With the proliferation of geospatial datasets driven by the rapid emergence of location-aware sensors, geospatial databases play a vital role in supporting geospatial applications. However, querying geospatial and temporal databases differs substantially from querying traditional relational databases due to the presence of geospatial topological operators and temporal operators. To bridge the gap between geospatial query languages and non-expert users, the geospatial research community has increasingly focused on developing NLIDBs for geospatial databases. Yet, existing research remains fragmented across systems, datasets, and methodological choices, making it difficult to clearly understand the landscape of existing methods, their strengths and weaknesses, and opportunities for future research. Existing surveys on NLIDBs focus on general-purpose database systems and do not treat geospatial and temporal databases as primary focus for analysis. To address this gap, this paper presents a comprehensive survey of studies on NLIDBs for geospatial and temporal databases. Specifically, we provide a detailed overview of datasets, evaluation metrics, and the taxonomy of the methods for geospatial and temporal NLIDBs, as well as a comparative analysis of the existing methods. Our survey reveals recurring trends in existing methods, substantial variation in datasets and evaluation practices, and several open challenges that continue to hinder progress in this area. Based on these findings, we identify promising directions for future research to advance natural language interfaces to geospatial and temporal databases.

==> search-method.tex <==
\section{Search Methodology}
%\textcolor{green}{Check if we are missing any steps for reproducibility. We need to add at least a few more content in this section for reviewer 2.}
This systematic review was conducted in accordance with the Preferred Reporting Items for Systematic Reviews and Meta-Analyses (PRISMA 2020) guidelines. The overall methodology followed a four-stage process consisting of: (i) systematic literature identification using predefined search queries, (ii) screening and eligibility assessment based on inclusion and exclusion criteria, (iii) full-text evaluation of shortlisted studies, and (iv) structured data extraction followed by qualitative synthesis.


\subsection{Search Strategy}
A comprehensive literature search was conducted across multiple digital libraries to identify relevant research on natural-language interfaces for spatial databases (NL2GeoSQL), spatial NLIDB systems, LLM-based spatial SQL generation, and multi-agent spatial question answering approaches. The databases we searched were: ACM Digital Library, IEEE Xplore, SpringerLink, Elsevier ScienceDirect, Web of Science, and Google Scholar. The search covered the period from January 2000 to December 2025, encompassing both traditional NLIDB systems and recent LLM-based approaches.

\hl{To ensure comprehensive retrieval, we constructed a Boolean search query by combining terms related to natural-language interfaces and spatial data. The final search string used for database retrieval is shown below.}

%\hl{The final search string was:}



% \begin{quote}
% \hl{("natural language interface" OR "natural language database interface" OR "NLIDB"} 
% \hl{OR "text-to-SQL" OR "NL2SQL" OR "natural language querying" OR "semantic parsing"} 
% \hl{OR "large language model" OR "LLM-based" OR "agent-based" OR "multi-agent")}
% \hl{AND}
% \hl{("geospatial" OR "spatial database" OR "GIS" OR "PostGIS" OR "SpatiaLite"} 
% \hl{OR "spatial SQL" OR "GeoSQL" OR "trajectory data" OR "spatial question answering")}
% \end{quote}


% \hl{The Boolean query was slightly adapted for each digital library to comply with database-specific syntax and indexing fields (e.g., title, abstract, and keywords).}


% \begin{table*}[!t]
% \centering
% \small
% \setlength{\tabcolsep}{6pt}
% \renewcommand{\arraystretch}{1.15}
% \caption{Search terms used for database retrieval.}
% \begin{tabular}{@{}p{0.28\textwidth} p{0.68\textwidth}@{}}
% \toprule
% \textbf{Concept} & \textbf{Search Terms} \\
% \midrule
% \textbf{Natural language interfaces} &
% ``natural language interface'', ``natural language database interface'', ``NLIDB'', 
% ``text-to-SQL'', ``NL2SQL'', ``natural language querying'', 
% ``query understanding'', ``semantic parsing'', 
% ``large language model'', ``LLM-based'', ``agent-based'', ``multi-agent'' \\[6pt]

% \textbf{Spatial and geospatial databases} &
% ``geospatial'', ``spatial database'', ``GIS'', ``PostGIS'', ``SpatiaLite'', 
% ``spatial reasoning'', ``spatial SQL'', ``GeoSQL'', ``trajectory data'', 
% ``spatial question answering'', ``geographic question answering'' \\
% \bottomrule
% \end{tabular}
% \label{tab:search_terms}
% \end{table*}


\vspace{5pt}
\noindent\fbox{%
  \begin{minipage}{\columnwidth}
    \textbf{\hl{The Final Search String}} \\
    \hrule \vspace{1mm}
    \raggedright
    \small
    \hl{("natural language interface" OR "natural language database interface" OR "NLIDB" OR "text-to-SQL" OR "NL2SQL" OR "natural language querying" OR "semantic parsing" OR "large language model" OR "LLM-based" OR "agent-based" OR "multi-agent")}\\
    \hl{AND}\\
    \hl{("geospatial" OR "spatial database" OR "GIS" OR "PostGIS" OR "SpatiaLite" OR "spatial SQL" OR "GeoSQL" OR "trajectory data" OR "spatial question answering")}
  \end{minipage}%
}




















In addition to database-driven searches, a complementary citation-based search strategy was employed to improve coverage. Specifically, backward citation searching was performed by examining the reference lists of key and highly relevant papers, while forward citation searching was conducted using Google Scholar to identify newer studies that cited these works. This iterative process helped identify additional relevant studies that may not have been captured through keyword-based searches alone.


The screening and management of all retrieved citations were conducted using the Rayyan web-based systematic review tool. The screening process consisted of four structured stages.

First, all citations retrieved from the electronic databases were imported into Rayyan and consolidated into a single library. Rayyan’s automated duplicate-detection functionality was then used to identify and remove redundant records across databases.

Next, the remaining citations were screened at the title and abstract level against predefined inclusion and exclusion criteria to remove irrelevant studies. Finally, the eligible articles were assessed through full-text review within Rayyan to determine their final inclusion in the review.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{images/prisma.eps}
    \caption{PRISMA 2020 flow diagram illustrating the study identification, screening, eligibility, and inclusion process.}
    \label{fig:prisma}
\end{figure}


\subsection{Inclusion Criteria}
Studies were included if they satisfied all of the following criteria:

\begin{enumerate}
    \item Addressed natural-language-to-GeoSQL generation or natural language query interpretation for spatial, spatiotemporal, or time-series data.
    \item Provided sufficient methodological detail to support technical understanding or replication.
    \item Were published as a peer-reviewed article, a full technical report, or a substantial arXiv manuscript.
    \item Were written in English and available in full text.
\end{enumerate}


\subsection{Exclusion Criteria}
Studies were excluded if they:

\begin{enumerate}
    \item Focused only on relational NLIDB without any spatial aspects.
    \item Addressed GIS visualization, mapping, or cartography without involving database querying.
    \item Discussed LLMs only at a conceptual level and did not include geospatial SQL.
    \item Did not provide a dataset, an evaluation, or had insufficient methodological information.
    \item Were posters, abstracts, or short preliminary papers.
\end{enumerate}

\subsection{Screening Process}
The study selection process followed the PRISMA 2020 guidelines and was conducted in two sequential stages: an initial screening of titles and abstracts, followed by a full-text eligibility assessment. A total of 90 records were retrieved from the electronic databases, including ACM Digital Library, IEEE Xplore, SpringerLink, and Elsevier ScienceDirect. In addition, 4 relevant studies were identified through manual searches on Google Scholar, resulting in 94 records in total.

All retrieved records were imported into the Rayyan web-based systematic review tool for citation management and screening. Rayyan’s automated duplicate-detection functionality was used to identify and remove redundant entries across databases, leading to the removal of 2 duplicate records and yielding 92 unique studies for screening.

In the first screening stage, titles and abstracts of the 92 records were reviewed against the predefined inclusion and exclusion criteria. During this phase, 57 studies were excluded because they did not fall within the scope of natural-language interfaces, spatial or spatiotemporal databases, or geospatial query generation.

The remaining 35 studies were subsequently retrieved in full and subjected to a detailed full-text eligibility assessment. Each article was evaluated based on relevance, methodological clarity, and alignment with the objectives of this review. Following this evaluation, 23 studies met all eligibility criteria and were included in the final qualitative synthesis. \hl{For each included study, key information was extracted using a structured template. The extracted attributes included dataset characteristics, query language, methodological approach, evaluation metrics, and system capabilities. This structured extraction enabled consistent comparison across ST-NLIDB systems.}
The overall flow of study identification, screening, eligibility assessment, and inclusion is summarized in Figure~\ref{fig:prisma}.



==> search-results.tex <==
\section{Results}
The results of this review take the evidence gathered from 21 studies that met the inclusion criteria. In this section, we present a structured summary of the main essence of these works, where we focus on the types of models that have been proposed, the datasets they used, the database systems they targeted, and the range of query types they addressed. To provide a clearer picture of how research in natural-language interfaces for spatial and spatiotemporal data has evolved, the findings are organized into several components, where we include an overview of the included studies, a detailed analysis of datasets, an examination of input–output feature design, and a taxonomy of methodological approaches. The subsections that follow describe these results in a systematic manner.

\subsection{Overview of Included Studies}
Based on the 21 studies included in this review, we observed a wide range of system designs, database platforms, and methodological choices. Earlier work mostly relied on rule-based parsing or handcrafted grammars, while more recent studies have started to adopt neural models, multi-agent LLM pipelines, and larger evaluation setups.

The studies also differ in the types of geospatial or spatiotemporal databases they target, such as PostGIS, Oracle Spatial, SECONDO, SpatiaLite, and a mix of synthetic or benchmark datasets. They also vary in the kinds of queries they handle; some focus only on spatial operators like within, intersects, or nearest neighbor, while others cover trajectory queries, spatiotemporal checks, or time-series comparisons. A smaller group deals with multi-step spatial reasoning and schema-aware SQL generation using LLM-based agents. Evaluation approaches range from basic qualitative examples to execution accuracy, semantic correctness, and ranking-based metrics.


Table~\ref{tab:included_studies} provides a summary of the included papers by listing the publication year, model type, database system, supported query types, and the evaluation metrics reported in each study.

\begin{table*}[!t]
\centering
\scriptsize
\caption{Summary of included studies with normalized evaluation metrics. \textcolor{red}{Does the table have all papers that you found later?}}
\label{tab:included_studies_normalized}
\begin{tabularx}{0.95\textwidth}{@{}p{0.09\textwidth}
p{0.06\textwidth}
p{0.27\textwidth}
p{0.21\textwidth}
p{0.27\textwidth}@{}}
\hline
\textbf{Paper} &
\textbf{Year} &
\textbf{Model Type} &
\textbf{DBMS} &
\textbf{Evaluation Metric (Normalized)} \\ 
\hline

\cite{chintaphally2007extending} &
2007 &
Menu-based NLI + rule-based grammar &
Oracle Spatial &
Qualitative / Human Evaluation \\

\cite{zhang2009natural} &
2009 &
Rule-based NLP + semantic parsing &
PostGIS &
Execution-Based Correctness \\

\cite{duntgen2009berlinmod} &
2009 &
Data generation and benchmark framework &
SECONDO &
Efficiency and Scalability \\

\cite{eldawy2015spatialhadoop} &
2015 &
MapReduce spatial framework (non-NLI) &
HDFS / SpatialHadoop &
Efficiency and Scalability \\

\cite{li2019spatialnli} &
2019 &
Seq2Seq GRU + spatial comprehension model &
Custom geospatial DB &
Interpretation / Translation Accuracy \\

\cite{wang2020nlmo} &
2020 &
Rule-based NLP + structured language generation &
SECONDO &
Execution-Based Correctness \\

\cite{wang2021nalmo} &
2021 &
Hybrid NLP + LSTM classifier + rules &
SECONDO &
Interpretation / Translation Accuracy; Precision-Oriented Correctness \\

\cite{xu2023grammar} & 
2023 &
Rule-based CFG, concept transformations &
No DBMS (abstract workflows) &
Qualitative / Human Evaluation \\

\cite{wang2023nalmo} &
2023 &
Hybrid semantic parsing + LSTM &
SECONDO &
Interpretation / Translation Accuracy \\

\cite{liu2023nalsd} &
2023 &
NLP + LSTM classifier + rule templates &
SECONDO &
Interpretation / Translation Accuracy; Efficiency and Scalability \\

\cite{ito2024clasp} &
2024 &
Contrastive learning (signal + text embeddings) &
N/A (time-series learning) &
Retrieval Quality (Ranking-Based); Qualitative / Human Evaluation \\

\cite{jiang2024chatgpt} &
2024 &
LLM prompting for spatial SQL &
PostGIS (NYC datasets) &
Execution-Based Correctness \\

\cite{khosravi2025questions} &
2025 &
Multi-agent spatial text-to-SQL &
PostGIS &
Qualitative / Human Evaluation \\

\cite{dohi2025retrieving} &
2025 &
Contrastive retrieval model &
N/A (TACO-based TS pairs) &
Retrieval Quality (Ranking-Based) \\

\cite{feng2025towards} &
2025 &
Multi-agent LLM + semantic search &
Vector DB + OSM layers &
Qualitative / Human Evaluation \\

\cite{houanl2sql} &
2025 &
LLM evaluation framework &
PostGIS (synthetic thematic DBs) &
Benchmark-Specific Composite Metrics; Structural / Syntactic Correctness \\

\cite{wang2025gpt} &
2025 &
GPT-based text-to-SQL with schema prompts &
SpatiaLite &
Execution-Based Correctness \\

\cite{yu2025monkuu} &
2025 &
LLM + dynamic schema mapping &
PostGIS + GeoQueryJP &
Structural / Syntactic Correctness \\

\cite{liu2025nalspatial} &
2025 &
NLP + LSTM type classifier + rule-based SLM &
SECONDO &
Execution-Based Correctness; Interpretation / Translation Accuracy \\

\cite{redd2025queries} &
2025 &
Multi-agent LLM (ReAct pipeline) &
SQL database (NYC/Tokyo check-ins) &
Execution-Based Correctness; Qualitative / Human Evaluation \\

\cite{wang2150nalmobench} &
2025 &
Text-to-EXE benchmark + evaluation (LLMs + baselines) &
SECONDO (executable language for MOD) &
Benchmark-Specific Composite Metrics; Execution-Based Correctness \\

\cite{zhang2025promassistant} &
2025 &
LLM + knowledge retrieval for text-to-PromQL &
Prometheus / PromQL &
Interpretation / Translation Accuracy; Precision-Oriented Correctness \\

\hline
\end{tabularx}
\end{table*}





% Another table goes here,



